Read Disturbance in High Bandwidth Memory: A Detailed Experimental Study on HBM2 DRAM Chips

We experimentally demonstrate the effects of read disturbance (RowHammer and RowPress) and uncover the inner workings of undocumented read disturbance defense mechanisms in High Bandwidth Memory (HBM). Detailed characterization of six real HBM2 DRAM chips in two different FPGA boards shows that (1) the read disturbance vulnerability significantly varies between different HBM2 chips and between different components (e.g., 3D-stacked channels) inside a chip, (2) DRAM rows at the end and in the middle of a bank are more resilient to read disturbance, (3) fewer additional activations are sufficient to induce more read disturbance bitflips in a DRAM row if the row exhibits the first bitflip at a relatively high activation count, (4) a modern HBM2 chip implements undocumented read disturbance defenses that track potential aggressor rows based on how many times they are activated. We describe how our findings could be leveraged to develop more powerful read disturbance attacks and more efficient defense mechanisms. We open source all our code and data to facilitate future research at https://github.com/CMU-SAFARI/HBM-Read-Disturbance.

==> sections/00_abstract.tex <==
\begin{abstract}

DRAM read disturbance is a significant and worsening safety, security, and reliability issue of modern DRAM chips that can be exploited to break memory isolation. Therefore, it is important to understand real DRAM chips' read disturbance characteristics. Two prominent examples of read-disturb phenomena are RowHammer and RowPress. Many existing DRAM modules of various form factors (e.g., DDR4) are vulnerable to RowHammer and RowPress. Unfortunately, no prior work extensively studies RowHammer and RowPress in modern high-bandwidth memory {(HBM)} chips{, which are commonly used in modern GPUs {and FPGAs}}. In this work, we experimentally demonstrate the effects of read disturbance and uncover the inner workings of undocumented in-DRAM read disturbance mitigation mechanisms in High Bandwidth Memory (HBM). 

%%%%% PRE HPCA REVIEWER A COMMENT %%%%%
% Our detailed characterization of six real HBM2 DRAM chips shows that 
% 1) the number of read disturbance errors (i.e., bitflips) and the number of row activations needed to induce the first read disturbance bitflip significantly varies between different HBM2 chips and different 3D-stacked channels, pseudo channels, banks, and rows inside an HBM2 chip, 
% 2) the DRAM rows at the end and in the middle of a DRAM bank exhibit significantly fewer read disturbance bitflips than the rest of the rows, 
% 3) it takes fewer additional activations to induce more read disturbance bitflips in a DRAM row if the row exhibits the first bitflip already at a relatively high activation count, and 4) HBM2 chips exhibit read disturbance bitflips with \emph{only two row activations} when rows are kept active for an extremely long time. 
%%%%% PRE HPCA REVIEWER A COMMENT %%%%%

Our detailed characterization of six real HBM2 DRAM chips shows that 
(1) the number of read disturbance errors (i.e., bitflips) and the number of row activations needed to induce the first read disturbance bitflip significantly varies between different HBM2 chips and different 3D-stacked channels, pseudo channels, banks, and rows inside an HBM2 chip.
\revlabel{Rev.A/C1}\reva{We observe that the variation in the average number of bitflips per DRAM row is more prominent across channels in some HBM2 chips than across all channels in all HBM2 chips.}
(2) The DRAM rows at the end and in the middle of a DRAM bank exhibit significantly fewer read disturbance bitflips than the rest of the rows.
(3) It takes fewer additional activations to induce more read disturbance bitflips in a DRAM row if the row exhibits the first bitflip already at a relatively high activation count. 
(4) HBM2 chips exhibit read disturbance bitflips with \emph{only two row activations} when rows are kept active for an extremely long time. 

We show that a modern HBM2 DRAM chip implements undocumented read disturbance defenses that can track potential aggressor rows based on how many times they are activated, and refresh their victim rows with every 17 periodic refresh operations. We draw key takeaways from our observations and discuss their implications for future read disturbance attacks and defenses. We explain how our findings could be leveraged to develop both i) more powerful read disturbance attacks and ii) more efficient read disturbance defense mechanisms.
%1) different 3D-stacked channels of HBM2 DRAM chips exhibit significantly different levels of {RowHammer} vulnerability, 2) the DRAM rows at the end of a DRAM bank {(rows with the highest addresses)} exhibit significantly lower {{RowHammer} vulnerability} than the rest of the rows, and 3) {a} modern HBM2 DRAM {chip} implement{s} {undisclosed} {RowHammer} defenses that {are triggered by} periodic refresh operations. 

%{We draw \param{X} key takeaways from our observations and discuss their implications for future {read disturbance} attacks and defenses. }

%\bscommentinline{4) something about rowhammer variation across 6 chips?}

%We discuss multiple directions for future work where we explain our plan to expand on the understanding of {RH} in 3D-stacked memories. \bscommentinline{For this version of the paper, not necessary to highlight future works, etc. So the last two sentences can be removed.}}I


\end{abstract}


==> sections/06_future_work.tex <==
\section{Future Work}
\label{sec:future_work}
{This work presents the results of our RowHammer characterization study on a real HBM2 DRAM chip.}
We plan to {present more insights into how RowHammer behaves in real HBM2 DRAM chips by strengthening our characterization study at least in the following directions}:

\noindent
\textbf{1) Testing more HBM chips}. We will repeat our experiments on a large{r} number of {HBM2} {chips} {to} {improv{e} the statistical significance of our observations}. \atbcomment{Remove this.} \bscommentinline{For me, the entire future work section can be removed. This version of the paper is supposed to be comprehensive so in theory nothing major should be remained for future.}

\noindent
\textbf{{2) More characterization} for each HBM chip}. {W}e plan to understand RowHammer's sensitivities to multiple other factors. We will investigate how {RH varies: 1) across different stacks in HBM2 chips, 2) based on the time an aggressor row remains active~\cite{orosa2021deeper}, 3) based on a richer set of data patterns used in initializing victim and aggressor rows, and 4) across different HBM2 voltage and temperature levels.} \atbcomment{Tricky. We need to justify why we do not study these (already in this paper) well.}

\noindent
\textbf{3) Investigating cross-channel interference.} {HBM2 chips 3D stack DRAM dies such that certain HBM channels are placed on top of each other. We will investigate if frequently accessing one or more \emph{aggressor channels} can induce bitflips or worsen the reliability characteristics of other \emph{victim channels}.}

%Due to the 3D-stacked nature of HBM, we suspect that continuous operation on a specific channel might cause some interference on a neighboring channel and thus affect its reliability.
% \begin{itemize} 
%     \item \textbf{Variation across different stacks.} Within the same HBM module, different stacks may have different levels of vulnerability to RowHammer.
%     \item \textbf{Impact of Aggressor Row Active Time.} Prior works \majdtodo{cite} contend that in DDRx the vulnerability of a DRAM victim row is also dependent on the aggressor row active time, which may also be true for HBM.
%     %We would therefore want to investigate such behavior for HBM.
%     \item \textbf{Cross-Channel Interference.} Due to the 3D-stacked nature of HBM, we suspect that continuous operation on a specific channel might cause some interference on a neighboring channel and thus affect its reliability.
%     \item \atb{\textbf{More data patterns.}}
%  \end{itemize}   

% \noindent
% \textbf{Process, voltage, and temperature \atb{(PVT)} variation.} As previously shown for DDRx, RowHammer bit flips can significantly vary under different PVT conditions [CITE]. We plan to verify this observations for HBMs as well. More specifically, one of the major concerns in HBM is the high temperatures at which it typically operates. We will address this problem by analyzing the behavior of RowHammer at different temperatures.

% \atbcommentside{Can be removed, kind of redundant after our "implications of spatial variation"}
% {We also plan to develop new RowHammer mitigations that primarily target HBM2 chips.}
% % but can also be used in other DRAM technologies.}
% %\atbcommentside{Put here speculatively.}
% Prior works propose many different RowHammer mitigations (e.g.,~\deterministicRowHammerDefenseCitations). {None of these techniques leverage the heterogeneity in the distribution of RH vulnerability across channels and across rows inside each channel. We plan to show the performance, energy, and chip area benefits of a defense mechanism that leverages this heterogeneity in HBM2 chips.}

%However, their efficiency for HBMs is not known. Considering the HBM-specific behavior of RowHammer bitflips, the associated  techniques may also need to be adapted accordingly. Our plan is to develop costly optimized RowHammer mitigation for specifically HBMs.
